Security in Automotive Networks: Lightweight Authentication and Authorization

With the increasing amount of interconnections between vehicles, the attack surface of internal vehicle networks is rising steeply. Although these networks are shielded against external attacks, they often do not have any internal security to protect against malicious components or adversaries who breach the network perimeter. To secure the in-vehicle network, all communicating components must be authenticated, and only authorized components should be allowed to send and receive messages. This is achieved using an authentication framework. Cryptography is widely used to authenticate communicating parties and provide secure communication channels (e.g., Internet communication). However, the real-time performance requirements of in-vehicle networks restrict the types of cryptographic algorithms and protocols that may be used. In particular, asymmetric cryptography is computationally infeasible during vehicle operation. In this work, we address the challenges of designing authentication protocols for automotive systems. We present Lightweight Authentication for Secure Automotive Networks (LASAN), a full lifecycle authentication approach. We describe the core LASAN protocols and show how they protect the internal vehicle network while complying with the real-time constraints and low computational resources of this domain. Unlike previous work, we also explain how this framework can be integrated into all aspects of the automotive lifecycle, including manufacturing, vehicle maintenance, and software updates. We evaluate LASAN in two different ways: First, we analyze the security properties of the protocols using established protocol verification techniques based on formal methods. Second, we evaluate the timing requirements of LASAN and compare these to other frameworks using a new highly modular discrete event simulator for in-vehicle networks, which we have developed for this evaluation.

==> content/authenticationFramework.tex <==
%!TEX root = ../lightweightAuthentication.tex
\section{Authentication Framework and Infrastructure}
\label{sec:AuthenticationFramework}
\numberofpages{3}
This section details the basic structure of the authentication framework, as well as the infrastructure that is required to build and run secure authentication for vehicles.
In addition to the protocols allowing the authentication between partners, an infrastructure to handle certificates and verify the system is required.
We compare the proposed approach and infrastructure for the lightweight authentication framework to other existing authentication frameworks, specifically in view of the special requirements in the automotive domain.
While our proposed framework is optimized for the automotive domain, it can be adapted to other distributed real-time systems with similar requirements as well.

% This section details the requirements of authentication for in-vehicle networks and evaluates existing frameworks, before proposing a lightweight framework for automotive real-time systems.
% While our proposed framework is optimized for the automotive domain, it can be adapted to other distributed real-time systems, too.
% \todophilipp{max 2 pages}
% \todophilipp{write introduction for this section}
% \todophilipp{find a better name for this section, maybe: Protocol}

% \todophilipp{
% - describe differences of setup key exchange \& runtime keys\\
% - establish key hierarchy (PK: OEM > GW/WS/Factory, Sym: ECU > Stream)\\
% - explain why we need two steps in the first place: multiple ECUs sharing keys, reducing messages (special case: multicast)\\
% - requirement: loose time synchronization
% - describe a bit more the underlying scheme: move expensive calculations to SM \& to setup time}

% \minisection{Setup/Update}
% \todophilipp{
% - describe initial key exchange\\
% - might be repeated (key update) at runtime in workshop (change of ECU) or over night\\
% - only allowed in programming mode of GW\\
% - explain chain of trust\\
% - explain certificate \& verification\\
% - mention validity of keys (lifetime/months/until further update)\\
% - where does the ECU key come from? => physically uncloneable function (PUF)\\
% - equation to estimate setup time required => put in experimental results?
% }
%
% \minisection{Runtime Protocol}
% \todophilipp{
% - describe new protocol\\
% - base description on needham-schroeder \& kerberos\\
% - explain differences to these \& why its sufficient\\
% - describe validitiy of keys (for real-time: when start of car, for non-real-time: when required)\\
% - equation to estimate stream setup time => put in experimental results?
% }
%
% \subsection{Scenario}
\subsection{Automotive Requirements}
Most \glspl{ECU} in vehicles have very limited memory and computational power.
To allow these devices to communicate securely, fast and efficient algorithms are required.
Symmetric cryptography is far less computationally demanding than asymmetric cryptography, and should hence be the method of choice.
However, these algorithms have the downside of requiring pre-shared keys.
For most approaches in the literature and industry, the distribution and management of keys is out of scope, not seldom leading to these keys being programmed into \glspl{ECU} during manufacturing.
This often leads to identical keys being used across a series of \glspl{ECU} and vehicles~\cite{koscher2010}.
This is a significant risk, as once a key is known, a whole series of vehicles might be susceptible to attacks.
With the number of individual vehicles per model reaching into the millions, the scaling effects of possible attacks are significant.
Thus, pre-programmed keys offer only limited security.

Additionally, not all \glspl{ECU} are connected directly or indirectly to outside networks such as the internet, nor should they be.
This adds additional complexity to the task of verifying certificate validity though an independent channel.
In case a device in the system, e.g. a security module or a workshop, behave maliciously or publicize their private key, their certificate will be revoked by the \gls{CA}.
This revocation has to be checked by communication partners to ensure communication is only established with legitimate devices.
This poses an additional challenge for asymmetric cryptography.

It is also worth noting that automotive networks are usually fixed at design time and, besides replacements of damaged \glspl{ECU}, nearly no changes to the architecture of the network occur at runtime.
Due to the highly distributed nature of the control tasks in vehicles, most of the communication of automotive networks are multicast or broadcast messages and only in some cases unicast messages are utilized to transmit information.
In the following, we will use the term \textit{message stream} to describe transmissions in the vehicle.
A message streams is defined as a topical message sent by one sender to one or multiple receivers.
Each message stream is uniquely identifiable via an ID and the message length and is transmitted periodically with the number of repetitions between one and infinite.
This definition describes all communication transmitted over in-vehicle networks as used today.

\subsection{Timed Efficient Stream Loss-Tolerant Authentication (TESLA)}
% \subsection{Existing Authentication Mechanisms}
% Multiple key exchange mechanisms have been proposed, optimized for different domains.
% In the following, we shortly evaluate a selection of mechanisms for their suitability in the automotive domain.
% \todophilipp{shorten}
% \minisection{TESLA}
To remedy the trade-off between symmetric and asymmetric cryptography, \gls{TESLA} was introduced to mimic asymmetric behavior with symmetric cryptography~\cite{perrig2005}.
All messages to be sent are encrypted with a locally generated key, which is subsequently published to the network.
A new key is generated after every broadcast of an earlier key.
Thus, all messages received before the key can be decoded on the target \gls{ECU}.
\gls{TESLA} tackles the issue of pre-programmed keys, but does not provide any control over which \glspl{ECU} can communicate on the bus nor does it provide any mechanism for reliably identifying \glspl{ECU}.
\gls{TESLA} can ensure that traffic is encrypted and can ensure that the sending \gls{ECU} can be identified, as only this \gls{ECU} has access to the correct encryption key (assuming unbreakable keys).
On the other hand, \gls{TESLA} is not capable of separating network traffic.
Every key is always shared between all participants on the bus, thus all participants can read every message.
Furthermore, access control to messages is not implemented.
To increase security, access control should be available.

As \gls{TESLA} does not provide any authentication mechanism and is based on symmetric encryption mechanisms, it is self-contained.
No support infrastructure is needed.

\subsection{Transport Layer Security (TLS)}
In contrast to \gls{TESLA}, TLS allows the sender and receiver to be authenticated using asymmetric cryptography \cite{dierks2008}.
\gls{TLS} development started as \gls{SSL} for use in internet applications and is the standard for authorization with HTTPS.
The authentication is performed based on asymmetric cryptography, using certificates and public/private key pairs.
During authentication, a symmetric key is exchanged, which is then used for encryption/decryption of data messages.
However, the asymmetric authentication and exchange can be computationally costly on embedded systems (see Section~\ref{sec:Results}).
Furthermore, \gls{TLS} does not support multicast/broadcast communication.
For every sender/receiver pair, a new key is generated.
Thus, to employ \gls{TLS} in the automotive domain, the encryption and sending of a message needs to be repeated for every receiving \gls{ECU}.
This is not efficient and feasible in automotive networks.

\gls{TLS} uses certificates to verify the identity of communication participants.
For correct verification of certificate validity, a connection to the \gls{CA} of the communication partner is required.
Via this connection, either \glspl{CRL} are downloaded or single certificates are checked, e.g., via protocols such as \gls{OCSP}.
This validation requires a communication channel, over which a secure connection can be established.
For inconsistent connections, \glspl{CRL} need to the saved for all communication partner \glspl{CA}.
The storage requirements for this can be quite large for embedded systems.
For single certificate validation, a secure connection to the \gls{CA} is required.
These connections are not and should not always be available in the automotive domain, if it means that \glspl{ECU} are connected to the internet.

\subsection{Kerberos}
Kerberos is an authentication framework for user authentication, built on symmetric cryptography~\cite{neuman2005}.
It allows devices to be authorized to use a service and enables distribution of keys using a pre-shared master key.
This pre-shared master key can be agreed upon using \gls{PKINIT}, an extension of the Kerberos framework.
\gls{PKINIT} uses asymmetric cryptography, allowing to negotiate a master key without any previous interaction \cite{zhu2006}.

Kerberos uses multiple servers, the \gls{AS} and the \gls{TGS}, together known as \gls{KDC}, to set up a connection to another device.
Multiple messages are required to handle this communication.
This is usually of limited importance, if user authentication is to be performed, as reaction times are much lower than message transmission times.
However, in real-time embedded systems, the larger number of messages and the induced delay make message stream setups infeasible.
Furthermore, as \gls{PKINIT} is based on asymmetric mechanisms, it requires the same certificate validation infrastructure as \gls{TLS}.
As shown above, this is not feasible in the automotive context.

\subsection{Lightweight Authentication Framework}
In \cite{mundhenk2015a}, we proposed to use a simplified version of the two-phase setup in Kerberos, adapted to the automotive context.
Kerberos is a highly flexible protocol to support the changing nature of consumer networks.
As automotive networks are of a more static nature, already fully defined at design time, we limited this flexibility and with this gained efficiency.
By limiting the flexibility to a minimal set for real-time systems and adjusting the underlying structure to the capabilities of automotive networks, we drastically reduced the amount of messages and data to be transmitted.
We reduced message exchanges by combining the \gls{AS} and \gls{TGS} into one system: The security module.
We further split the phases of the protocol into different periodical phases in the life cycle of the vehicle, allowing us to reach real-time behavior.

\begin{figure}
	\centering
	\includegraphics[width=\hsize]{./diagrams/Overview.pdf}
	\caption{In our framework, every ECU is authenticated against the security module (1a-1c).
	Subsequently, the ECU can request the keys for a message stream (2.1a-2.1b) and start transmitting (3.1).
	If the ECU is to start receiving a message stream, it is notified by the security module with the message stream key (2.2b) before it receives the stream (3.2).}
	\label{fig:overview}
\end{figure}

% \minisection{Two Phase Authentication}
We used the two-phase authentication of Kerberos as shown in Fig.~\ref{fig:overview}:
\begin{enumerate}
	\item ECU authentication (asymmetric)
	\item Stream authorization (symmetric)
\end{enumerate}
We proposed to employ the asymmetric phase of the framework for \gls{ECU} authentication.
This can be performed periodically, while the vehicle is not in operation.
The interval depends on the strength of the algorithm used for symmetric cryptography.
The interval needs to be shorter than the time it would take to break the key with potentially available devices.
The symmetric phase of our framework is used for stream authorization and is performed as required.
By receiving the key to a message stream from the security module, an \gls{ECU} is granted the right to access the stream and communicate with other participants in the network.
Depending on the real-time requirements of the stream, this step can be performed either at vehicle start-up, or when the setup of a message stream is required.

In this work, we formally verify the proposed protocol and improve the protocol in multiple places.
We improve the \gls{ECU} authentication, disabling man-in-the-middle attacks at vehicle reboot.
This is detailed in Section~\ref{sec:Verification}.

As our proposed approach uses asymmetric encryption, we also require a certificate creation and validation architecture.
Due to the special requirements of the automotive domain, we employ a combination of \glspl{CRL} and single certificate validation to most efficiently handle validity checks.
This is detailed in Section~\ref{sec:CRL}.
Certificates are created at manufacturing time of the devices.
This process is detailed in Section~\ref{sec:Scenarios}.
There, we further detail abnormal situations the vehicle might experience, such as workshop situations, including replacements of \glspl{ECU}, which to the best of our knowledge, presents an unsolved problem until today.

% \todophilipp{then: detailed contribution}

% This section addresses the challenges described in Section~\ref{problemDescription} in detail and describes our proposed solution.
% To enable the encryption and key-based security mechanisms described in literature, while avoiding pre-programmed keys, we borrow methods from existing protocols and adapt these for use in automotive real-time systems.
% The general concept is based on the Kerberos protocol with \gls{PKINIT} for initial key distribution.
% We exploit the specific structure of automotive networks, mainly the multicast behavior.
% In automotive networks, messages are mostly transmitted from one sender to multiple receivers.
% To keep the bus utilization low, we propose to share one symmetric key between the sender and all receivers of a stream $s$.
% This way, messages to not need to be sent multiple times with different keys to different receivers.e
% \glspl{ECU} are authenticated against a security module, which also authorizes access to message streams.
% Communication participants are not authorized against each other, but always against a central security module.
% This is possible as the car network is mostly fixed in its hardware and message structure.
% Authentication against the security module lowers the number of messages required and additionally allows to control the security of the vehicle from one central element, the security module.
% This setup is used to generate a key hierarchy in which each key lower in the hierarchy can be retrieved by a key higher up in the hierarchy: $k_{e,\mathrm{priv}}/k_{e,\mathrm{pub}} > k_{e,\mathrm{sym}} > k_{s}$.
% The asymmetric encryption is based on certificates which we assume to be unforgeable, e.g. by means of sufficiently long keys.
% The required keys for the asymmetric handshake, as well as the \gls{ECU} key should be generated based on a \gls{RNG} which can be coupled with a \gls{PUF} \cite{lim2005}.
% This way, true random numbers are generated which can not be reproduced by attackers using identical hardware.
% While the network architecture can be of any kind, a security module is required in the network, authenticating and authorizing \glspl{ECU} and message streams.
% From a security perspective, it is beneficial to implement such a security module at a central point of the network, e.g. a central gateway.
% In this case, the knowledge of authorized message streams can be used to forward or block streams, similar to a firewall.
% From a performance perspective, the security module should be equipped with sufficient resources to store all keys and also hardware support for public-key cryptography.
% Should no hardware support for public-key cryptography be available, the setup times will increase significantly.

% For higher security, the keys used for encryption and decryption are required to be as long as possible.
% This holds for asymmetric encryption, as well as symmetric encryption:
% \begin{equation}
% 	\label{equ:keyLenAsym}
% 	\begin{split}
% 		\argmax_{\mathrm{l} \in \{2^n | n\geq9, n\in \mathbb{N}\}} \{c = \epsilon^{a}_{d}(t,k) | k=(v,l)\}
% 	\end{split}
% \end{equation}

% \begin{equation}
% 	\label{equ:keyLenSym}
% 	\begin{split}
% 		\argmax_{\mathrm{l} \in \{128,196,256\}} \{c = \epsilon^{s}_{d}(t,k) | k=(v,l)\}
% 	\end{split}
% \end{equation}
% The steps of the exchange are explained in more detail in the following.


==> content/crls.tex <==
%!TEX root = ../lightweightAuthentication.tex
\section{Certificate Validation}
\label{sec:CRL}
\numberofpages{1}
The security of asymmetric cryptography relies on the security of the distributed certificates.
This security is not static.
If a certificate containing a private key of an entity is stolen or purposely distributed with malicious intent, the certificate can no longer be assumed secure.
As the private key is known, any participant can impersonate the entity of the leaked certificate.
Participants need to be able to recognize the compromised certificate to ensure no communication is established with this potentially compromised element.
Two approaches are commonly used to check the validity of certificates:
(1) Lists of invalid certificates are collected in Certificate Revocation Lists (CRLs) \cite{cooper2008} or (2) the validity of a single certificate is checked with the help of a server, e.g. with \gls{OCSP} \cite{santesson2013}.
Both approaches have advantages and disadvantages.
While \glspl{CRL} require a larger amount of memory, single certificate checks require a secure connection for validation.
For the highest efficiency, we combine both approaches.
We select between \glspl{CRL} and single certificate checks depending on the number of devices potentially to be verified and the situation of the verifying device.
The different use cases are shown in Table~\ref{tab:validation}.
% Information for these insecure certificates is collected in \glspl{CRL} \cite{cooper2008}.
% A \gls{CRL} is a list of certificates that have lost their validity, created and signed by the issuing authority.
% \glspl{CRL} need to be distributed to all communication participants to ensure the security of their communication.
% These lists can reach rather large sizes, often in the size of megabytes for each \gls{CA}.
% As generally the \glspl{CRL} of multiple \glspl{CA} are required to cover all communication participants, the amount of data to be transmitted and stored is no insignificant for an embedded system.
% Small embedded systems can be limited in memory to the hundred kilobytes range.
% On the internet today, \glspl{CRL} are slowly replaced by the \gls{OCSP} \cite{santesson2013}.
% The \gls{OCSP} avoids downloads of large lists and instead checks the status of single certificates online.
% For this however, a connection to the \gls{OCSP} responder (generally the \gls{CA}) is required.
% In automotive settings, such a connection can not be guaranteed.
% We thus need to optimize the distribution of \glspl{CRL}, to reach an efficient and secure handling of revoked certificates.

\minisection{Single validation (asynchronous)}
An \gls{ECU} validating the certificate of a security module only requires validation of one device.
It would thus be inefficient to transmit revocation lists to this \gls{ECU}.
Instead, we use single certificate checking to check the certificate against the issuing \gls{CA}.
The protocol used for this could be \gls{OCSP}, which can be used with minor adjustments for the automotive domain.
This checking however, is done asynchronously.
With a dynamic device, such as a vehicle, we can not always guarantee an internet connection.
Thus, the validation of the security module certificate is performed periodically, based on key and algorithm strength, internet connection and \gls{ECU} performance.
This can either be performed via a built-in cellular connection or other means of internet access, e.g. at a charging station for electric vehicles.
The outcome of this validation is stored until the next periodical validation.

\minisection{Single validation (synchronous)}
In some situations, a connection to the \gls{CA} can be established.
This is for example the case for workshop situations, in which the car can establish an internet connection through the connection to the workshop.
Here, a secured connection, such as specified in \gls{OCSP} is of particular importance, to avoid man-in-the-middle attacks by the workshop.
In these situations, we use a synchronous validation of the certificate.
Thus, we only launch the validation whenever it is required, e.g. when a workshop tries to authorize against the security module.
This single check is also performed when the workshop tries to authorize against an \gls{ECU}.
In this case, a single validation is performed by the \gls{ECU} with the help of the security module, which stores the relevant \gls{CRL} for workshop devices.

\minisection{CRL}
In some situations, the \glspl{CRL} are required to be available at all times.
This is for example necessary, if the security module validates \gls{ECU} certificates.
As more than one certificate is validated here, it makes sense to save the \gls{CRL}, specifically filtered for the car.
This filtering is performed on the side of the \gls{CA} and only the \gls{CRL} relevant to a specific vehicle is transmitted to and saved on the security module.
Due to the abundant storage on workshop computers, \glspl{CRL} can also be used here to verify security module and \gls{ECU} certificates.

% \subsection{CRL Format}
% \label{sec:CRL_format}
% \todophilipp{remove?}
% To facilitate certificates, we create a tree of trust along the lines of the structure of automotive \glspl{OEM}
% This tree of trust is shown in Figure~\ref{ToDo}.

% \glspl{CRL}, as used on the internet today store data quite efficiently.
% Besides information about the issuer of the \gls{CRL}, the entries of the \gls{CRL} contain only the serial number of the certificate to be revoked and the revocation date, sometimes additionally a revocation reason is given.
% As \glspl{ECU} generally do not have to analyze previous communication, we drop the revocation date from the list and simply provide a list of serial numbers for revoked certificates.
% We further also do not require a reason for certificate revocation, so we also drop this field and only save the certificate serial number in the \gls{CRL}.

% \subsection{Filtering}
% \label{sec:CRL_filtering}
% To save as much memory as possible, a filtering is introduced to only transmit relevant \glspl{CRL} entries.
% This filtering is performed by the \gls{CA}.

With these three validation options, the amount of memory and transmissions is reduced to a minimum.
Periodic checks of certificates are possible and invalid certificates can be detected, thus securing all communication between all participants.

\begin{table}
\tbl{The verifying device and the device to be verified determine the verification method, as well as the Certificate Authority (CA) to verify against.}{
\centering
    \begin{tabular}{cc|cc}
	    \toprule
	    \textbf{Verifier} & \textbf{Device to verify} & \textbf{Verification method} & \textbf{verifying CA} \\
	    \midrule
	    ECU & security module & single validation (asynchronous) & CA of security modules \\
	    security module & ECU & CRL & CA of ECUs \\
	    ECU & workshop & single validation (synchronous) & security module \\
	    security module & workshop & single validation (asynchronous) & CA of workshops \\
	    workshop & security module & single validation/CRL & CA of security modules \\
	    workshop & ECU & single validation/CRL & CA of ECUs \\
	    \bottomrule
    \end{tabular}}
\label{tab:validation}
\end{table}

==> content/design.tex <==
%!TEX root = ../lightweightAuthentication.tex
\section{Design}
\label{sec:Design}
In this section, we introduce the \gls{ECU} authentication and stream authorization approaches in detail.
Our explanations follow along \cite{mundhenk2015a}.
Some of the messages here have additional components, compared to \cite{mundhenk2015a}.
These have been determined as required in the verification and implementation of our framework and are required for increased security or lower latency.
The components are explained accordingly.

\subsection{Terminology}
To understand the lightweight authentication, the following terminology is required.
We denote an \gls{ECU} as $e$, sending a set of streams $S_e$ to a set of receiving \glspl{ECU} $R_e$.
In turn, a stream $s \in S_e$ is identified by the sending \gls{ECU} $e$, a set of receiving \glspl{ECU} $R_s$ and a set of message instances $M_s$: $s=(e,R_s,M_s)$.
A message instance $m \in M_s$ is assigned to a stream $s$ and carries a payload $o$.
The security module of the system is denoted as $y$.
A timestamp on device $d$ is denoted as $\omega_d$ and a random number as $\rho$.
A nonce $n$ is a unique random number $\rho$ within the accuracy of one timestamp.
Together, timestamp and nonce shall be unique over the lifetime of the vehicle, while minimizing the storage required for nonces.
A key is denoted as $k$ and identified by its value $v$ and its length $l$.
We further define a hashing function for message $m$ on device $d$ as $h_d(m)$.
A parameter to determine if the system is running is defined as $\theta \in \{0,1\}$ and a function $\alpha(e,s) \in \{0,1\}$ determines if an \gls{ECU} $e$ has access to the stream $s$ (1) or not (0).
The time required to execute a function $x$ is defined as $\tau_x$.
An action $z$ is triggered, if a condition $i$ is fulfilled: $i \rightarrow z$.

\subsection{ECU Authentication}
\label{sec:Design_ECUAuthentication}
% \minisection{Key Exchange}
The key exchange used for \gls{ECU} keys is based on the \gls{PKINIT} protocol for Kerberos.
\gls{PKINIT} has been chosen for its conciseness.
This reduces the required time and bandwidth for the authentication.
The \gls{ECU} authentication is illustrated in Fig.~\ref{fig:overview} and described in the following.
% First, we define the authentication mechanism for \glspl{ECU}.
This mechanism facilitates the initial key exchange between the \gls{ECU} and the security module, and is based on asymmetric cryptography.
Secure asymmetric cryptography is generally a computational expensive task.
This holds especially for software implementations without hardware support, as it will be the case on most \glspl{ECU}.
Thus, this \gls{ECU} authentication needs to be executed when the vehicle is not in use to not interfere with the real-time capabilities of the system.

\begin{figure}
	\centering
	\includegraphics[width=\hsize]{./diagrams/Overview.pdf}
	\caption{In our framework, every ECU is authenticated against the security module (1a-1c).
	Subsequently, the ECU can request the keys for a message stream (2.1a-2.1b) and start transmitting (3.1).
	If the ECU is to start receiving a message stream, it is notified by the security module with the message stream key (2.2b) before it receives the stream (3.2).}
	\label{fig:overview}
\end{figure}

\minisection{Authentication Mechanism}
To describe \gls{ECU} authentication, we define a set of keys for device $d$, consisting of a public key $k_{d,\mathrm{pub}}$ and a private key $k_{d,\mathrm{priv}}$.
We further define an asymmetric encryption function $\epsilon^a$ for device $d$, that translates clear text $t$ into cipher text $c$ with key $k$, such that $c = \epsilon^a_d(t,k)$.
Accordingly, we define an asymmetric decryption function $\delta^a$ for device $d$, that translates cipher text $c$ into clear text $t$ with key $k$, such that $t = \delta^a_d(c,k)$.
For authentication, we further require the certificate $f_d$ for device $d$ and a function $\phi_{d_{1}}(f_{d_{2}}) = \{0,1\}$ to verify the certificate $f_{d_{2}}$ on device ${d_{1}}$.

As shown in Fig.~\ref{fig:overview}, three steps are required to authenticate an \gls{ECU}.
First, the security module needs to make itself known and authenticate to all \glspl{ECU}.
Second, each \gls{ECU} authenticates to the security module and requests a symmetric key.
Third, the security module permits the requesting \gls{ECU} to access the bus by sending a confirmation message to this \gls{ECU}.
These steps are described in the following:

\begin{enumerate}[(a)]
	\item
Advertisement by the security module (Fig.~\ref{fig:overview}~(1a)):
The security module $y$ advertises its certificate to every \gls{ECU} on the bus at startup with message $m_a$.
This certificate is required to be signed by the appropriate \gls{CA} (see Section~\ref{sec:CRL}).
\begin{align}
\label{equ:ad}
	\theta \rightarrow m_a \ \mathrm{with} \ m_a \in M_{s}^{a}, \ s = (y, \{e\},M_{s}^{a}), \ o = f_{y}
\end{align}
The authentication of the security module $y$ is achieved by presenting a valid security certificate $f_y$ to \gls{ECU} $e$.
The certificate (including the public-key) of the security module is broadcast on the network unencrypted.
Each \gls{ECU} has a pre-programmed list with the certificates of the intermediary \glspl{CA} and the root \gls{CA}.
With this data, the certificate of the security module can be verified.
It is to be noted that the programmed list should be regularly updated with a \gls{CRL} (see Section~\ref{sec:CRL}).
	\item
Registration of the \gls{ECU} (Fig.~\ref{fig:overview}~(1b)):
On successful verification of the security module ($\phi_{e}(f_y) = 1$), the \gls{ECU} transmits its registration message $m_r$, including its own certificate $f_e$ and the newly generated \gls{ECU} key $k_{e,\mathrm{sym}}$.
The key, a timestamp $\omega_{e}$ and a nonce $n$ are encrypted with the public key of the security module $k_{y, \mathrm{pub}}$ and can thus only be decrypted by the security module.
Note that the ECU identifier is contained in the certificate $f_e$ and thus does not need to be added separately to the message:
\begin{align}
\label{equ:register}
	\phi_{e}(f_y) &\rightarrow m_r\\
	\mathrm{with} \ m_r &\in M_{s}^{r},\ s = (e, \{y\}, M_{s}^{r}),\nonumber\\
	o &= (\epsilon^{a}_{e}((e, y, k_{e, \mathrm{sym}}, n, \omega_{e}), k_{y, \mathrm{pub}}), \epsilon^{a}_{e}(h(e, y, k_{e, \mathrm{sym}}, n, \omega_{e}),k_{e, \mathrm{priv}}), f_{e})\nonumber
\end{align}
In comparison to \cite{mundhenk2015a}, we added an additional hash of the data to be transmitted, encrypted with the private key of $e$.
This allows the security module to verify the authenticity of the sender as being \gls{ECU} $e$ (see Section~\ref{sec:Verification}).
We also added the identifier of \gls{ECU} $e$ to avoid attacks following Dolev-Yao adversary model (see Section~\ref{sec:Verification}).
Without these two additions man-in-the-middle attacks on the authentication protocol are possible, defeating the purpose of the protocol.

	\item
Confirmation of the security module (Fig.~\ref{fig:overview}~(1c)):
Upon receiving the registration message, the security module verifies the sender of the message.
This is verified by decrypting the received hash from $m_{r}$ and comparing it to the hash of the received elements.
The elements have been received separately in $m_{r}$ and need to be decrypted with the private key of the security module $k_{y,\mathrm{priv}}$.
Additionally, the certificate of the sender is verified and, in the case of successful verification ($\phi_{y}(f_e) = 1$), the security module saves the \gls{ECU} key and sends a confirmation message $m_c$ to the \gls{ECU}.
This message contains the \gls{ECU} identifier, encrypted with the newly exchanged symmetric \gls{ECU} key:
\begin{align}
\label{equ:confirm}
	\delta^{a}_{y}(\epsilon^{a}_{e}(h(y, &k_{e, \mathrm{sym}}, n, \omega_{e}),k_{e, \mathrm{priv}}), k_{e, \mathrm{pub}})=h(y, k_{e, \mathrm{sym}}, n, \omega_{e})) \wedge \phi_{y}(f_e) \rightarrow m_c\\
	\mathrm{with} \ m_c &\in M_{s}^{c}, \ s = (y, \{e\}, M_{s}^{c}), \ o = (e, y, \epsilon^{s}_{y}((e, n, \omega_{y}), k_{e, \mathrm{sym}}))\nonumber
\end{align}
In comparison to \cite{mundhenk2015a}, an additional \gls{ECU} identifier $e$ has been introduced to identify the receiving \gls{ECU} and minimize unnecessary computational overhead for decryption.
Without this identifier, each received message first needs to be decrypted, which might not be possible, as every \gls{ECU} uses different keys.
This would increase the time for \gls{ECU} authentication manifold.
\end{enumerate}
Besides the shown security validations, the sanity of timestamps and integrity of the timestamp/nonce combination needs to be validated for every message.

This concludes the \gls{ECU} authentication.
In order to transmit messages via an encrypted channel, the \gls{ECU} needs to request a stream key from the security module.
This is handled via the stream authorization, as described in the following.
% To exchange the symmetric \gls{ECU} key, the security module needs to be in programming mode.
% This mode can only be activated by a certified factory or workshop, verified via a certificate.
% The additional programming mode is required to ensure that a replaced or compromised \gls{ECU} can not simply overwrite the key of an earlier \gls{ECU}, even if it presents a valid certificate.

% \minisection{Latency}
% The latency $\tau_{\mathrm{setup}}$ introduced by \gls{ECU} authentication is only of limited relevance, as this is performed at times when the car is not in operation, such as in a factory or workshop.
% However, for completeness, we can define the latency based on the time $\tau_x$ required for the functions in Equations~\eqref{equ:ad}, \eqref{equ:register} and \eqref{equ:confirm}, summing up to the full latency of:
% \begin{equation}
% \label{equ:t_setup}
% \tau_{\mathrm{setup}} = \tau_{\phi_{e}} + \tau_{n} + \tau_{\epsilon_{e}^{a}(t,k_{\mathrm{pub}})} + \tau_{\phi_{y}} + 3 \cdot \tau_{tx}
% \end{equation}

% This setup time omits minor latencies, such as message passing within the \gls{ECU} and security module.
% As shown in Section~\ref{experimentalResults}, without hardware support for public key encryption, it holds:
% To verify a certificate, the signature of the certificate must be decrypted and the contained hash compared to a locally computed hash of the certificate:
% While the certificate also needs to be compared to the \glspl{CRL}, which requires its own network communication, we omit this step and assume that all required \glspl{CRL} are available locally.
% The efficient distribution and handling of \glspl{CRL} should be investigated in further research.
% Thus, we define:
% \begin{equation}
% \label{equ:t_verify}
% \tau_{\phi_{e}} = \tau_{\delta_{e}^{a}(c,k_{\mathrm{pub}})} + \tau_{h_{e}(m)} + \tau_{\mathrm{comp}_{e}}
% \end{equation}

% For the RSA algorithm, it holds that
% \begin{equation}
% \label{equ:rsaEqu1}
% \tau_{\epsilon_{d}^{a}(t,k_{\mathrm{pub}})} = \tau_{\delta_{d}^{a}(c,k_{\mathrm{pub}})}
% \end{equation}
% and
% \begin{equation}
% \label{equ:rsaEqu2}
% \tau_{\epsilon_{d}^{a}(t,k_{\mathrm{priv}})} = \tau_{\delta_{d}^{a}(c,k_{\mathrm{priv}})}.
% \end{equation}

% \minisection{Key Lifetime}
% As the \glspl{ECU} cannot be assumed to have access to a \gls{CA} at runtime, the update of \gls{ECU} certificates cannot be performed easily.
% Thus, the certificates and the public and private keys have to be valid for the lifetime of the \gls{ECU}.
% However, the defined automotive certificate format has a validity field, allowing certificate lifetime to be limited in future revisions of the system.

% % The initial key exchange for all symmetric \gls{ECU} keys is based on an asymmetric exchange.
% The public and private \gls{ECU} keys are generated on the \gls{ECU} itself and certified by the \gls{OEM}.
% The certification and first key exchange is performed under the control of the \gls{OEM} when manufacturing the vehicle.
% The exchange might need to be repeated when repairing the vehicle and exchanging \glspl{ECU}.
% Additionally, a periodical repetition of the exchange should be considered, reducing the attack surface by periodically renewing the symmetric \gls{ECU} keys.
% As it cannot be assumed that all \glspl{ECU} have hardware support for asymmetric cryptographic functions, the functions might need to be implemented in software (see Fig.~\ref{fig:ecu}).
% As this is considerably slower than a hardware implementation (see Section~\ref{experimentalResults}), an optimal update cycle needs to be found, not weakening security while keeping \gls{ECU} load low.
% Having two separate phases allows this to be optimized with respect to the specific requirements of the vehicle.

% \minisection{Certificate Hierarchy}
% The \gls{ECU} key exchange mechanism is based on established asymmetric cryptographic frameworks.
% Each \gls{ECU} generates a public and private key for itself in the production process.
% The keys are certified in a chain of trust, to be established by the \gls{OEM}.
% % \begin{figure}
% % 	\centering
% % 	\includegraphics[width=\hsize]{./diagrams/KeyHierarchy.pdf}
% % 	\caption{The chain of trust shows which entities are certified by which Certificate Authorities (CAs).
% % 	To guarantee efficient processing, the chain of trust should not exceed a length of 4.
% % 	By trusting a CA higher in the chain, trust can propagate efficiently through the chain.}
% % 	\label{fig:keyHierarchy}
% % \end{figure}
% At the root of the certificate hierarchy is the root \gls{CA} of the \gls{OEM} which certifies all intermediary \glspl{CA}.
% The root \gls{CA} should not directly certify any devices, but instead certify intermediary \glspl{CA} which in turn certify devices.
% In this way, potential misuse of the private key of the root \gls{CA} is minimized.
% The intermediary \glspl{CA} are represented by factories and workshops.
% A second intermediary tier could be introduced to reflect the geography and/or organizational structure of the \gls{OEM}, if required.

\subsection{Stream Authorization}
\label{sec:Design_StreamAuthorization}
After \glspl{ECU} authenticate themselves with the security module and set symmetric \gls{ECU} keys, the \glspl{ECU} can request initiations of message streams.
All message streams and stream keys in the system are administered by the security module.
Sending and receiving \glspl{ECU} need to request the key for each message stream from the security module.
This module authorizes access to message streams; authentication between sending and receiving \glspl{ECU} for a stream is not required.
The stream setup is performed when a message stream is required, or, if the real-time requirements are stricter than the stream setup time, considerably in advance, e.g., at the start of the vehicle.
% Fig.~\ref{fig:streamAuthentication} illustrates stream authorization.
% \begin{figure}
% 	\centering
% 	\includegraphics[width=\hsize]{./diagrams/StreamAuth.pdf}
% 	\caption{To initiate a message stream, the sending ECU $e_1$ requests the stream key from the security module $y$ with message $m_q$ (2a).
% 	If the sending ECU is allowed to access the stream, the security module grants stream access first to all receiving ECUs (2b1-2b2) and last to the sending ECU (2b3).
% 	Subsequently, the sending ECU can start transmitting the message stream $s_{i}$ (3).}
% 	\label{fig:streamAuthentication}
% \end{figure}

\minisection{Authorization Mechanism}
For stream authorization, we define a symmetric key $k_{\mathrm{sym}}$ and two functions $\epsilon^s$ and $\delta^s$ for encryption and decryption, such that $c = \epsilon_{d}^{s}(t,k_{\mathrm{sym}})$ and $t = \delta_{d}^{s}(c,k_{\mathrm{sym}})$ for clear text $t$ and cipher text $c$ on device $d$.
\ \\
The stream can only be established after the \gls{ECU} receives the confirmation message $m_c$ for \gls{ECU} authentication (see Fig.~\ref{fig:overview} (1c)).
It is usually established when a message $m$ is requested to be sent.
The sending \gls{ECU} $e$ can then request a key from the security module $y$, allowing access to the stream.
The request message $m_q$ contains the identifier of the requested stream $s_{i}$, the identifier of the requesting \gls{ECU} $e$, as well as a timestamp $\omega_e$ and a nonce $n$ to protect against retransmissions.
The content of the message $m_q$ is encrypted with the \gls{ECU} key $k_{e, \mathrm{sym}}$:
	\begin{align}
	\label{equ:stream}
	% \begin{align}
		m_c \wedge m &\rightarrow m_q\\
		\mathrm{with} \ m_q &\in M_{s}^{q}, \ s = (e, \{y\}, M_{s}^{q}),\nonumber\\
		o &= (e, \epsilon^{s}_{e}((e, s_{i}, n, \omega_e), k_{e, \mathrm{sym}}))\nonumber
	% \end{align}
	\end{align}
In contrast to \cite{mundhenk2015a}, an additional unencrypted sender identifier $e$ has been introduced to simplify key selection for decryption on the security module.
If the received request message $m_q$ can be successfully decrypted with the \gls{ECU} key $k_{e, \mathrm{sym}}$ and the requesting \gls{ECU} $e$ is allowed access to the stream $s_{i}$ ($\alpha(e, s_{i}) = 1$), the security module $y$ assigns a key $k_{s_{i}, \mathrm{sym}}$ to the stream.
This key is forwarded to all receiving \glspl{ECU} $\tilde{e} \in R_{s_{i}}$, as well as the requesting sending \gls{ECU} $e$.
% As the security module is aware of all \glspl{ECU} being part of the stream, the key is also distributed to all receiving \glspl{ECU}.
This way, it is ensured that all receivers have access to the data as soon as it is sent:
	\begin{align}
	\label{equ:grant}
	% \begin{align}
		m_q \wedge (\delta_{y}^{s}(m_q, k_{e, \mathrm{sym}}) &= (e, s_{i}, \omega_e, n))\\
		\wedge (\omega_e \leq \omega_y) \wedge \alpha(e, s_{i}) &\rightarrow \forall \tilde{e} \in \{R_{s_{i}}, e\}: m_g\nonumber\\
		\mathrm{with} \ m_g &\in M_{s}^{g}, \ s = (y, \tilde{e}, M_{s}^{g}),\nonumber\\
		o &= \epsilon^{s}_{y}((\tilde{e}, s_{i}, k_{s1, \mathrm{sym}}, n_i, \omega_y), k_{\tilde{e}, \mathrm{sym}}),\nonumber\\
		n_i = \rho : \rho \notin &\bigcup_{l} \rho_{l}, l=\{0..i-1\}\nonumber
	% \end{align}
	\end{align}
% To verify that received messages are not replays of older messages, loose time synchronization should be available in the network.
% Alternatively, the security module can safe previously received timing values $\omega_e$.

% \minisection{Latency}
% Similarly to the latency for \gls{ECU} authentication, we can calculate the upper bound of the latency for stream authorization by adding the latencies of all functions required in Equations~\eqref{equ:stream} and \eqref{equ:grant}.
% In the case of $x$ \glspl{ECU} participating in the stream, the latency can be defined as:
% \begin{align}
% \label{equ:t_auth}
% \tau_{\mathrm{stream}} = \ &(x+1) \cdot \tau_{\epsilon^{s}_{e}(t,k_{\mathrm{sym}})} + 2 \cdot \tau_{\delta^{s}_{e}(t,k_{\mathrm{sym}})}\\
% + &(x+1) \cdot \tau_{n} + (x+1) \cdot \tau_{tx}\nonumber
% \end{align}

% All values are assumed to be equal across all \glspl{ECU} and the security module, as hardware support for random number generators and symmetric encryption/decryption is assumed.

% \minisection{Key Lifetime}
% The key lifetime is heavily dependent on the required setup speed for message streams.
% We can broadly separate message streams into two categories:\\
% % \begin{itemize}
% 	% \item
% \textit{Real-Time Traffic:}
% As real-time traffic has the most stringent requirements regarding timing, message streams should already be established when the message needs to be sent.
% This can be achieved by setting up message streams at vehicle start-up.
% Thus, the keys required for real-time streams are already present in the \glspl{ECU}, when the real-time message needs to be transmitted.\\
% 	% With such prepared streams, the only overhead introduced to the message transmission is determined by the delay caused by treating the message to be secure.
% 	% This treatment could be encryption, Message Authentication Codes (MACs), or similar.
% 	% \item
% \textit{Non-Real-Time Traffic:}
% For non-real-time traffic, the stream setup can be slower than for real-time traffic, as long as it occurs in defined intervals.
% If at any point in the transmission, a human is involved (e.g. by pressing a button), the human reaction time defines an upper bound to the latency.
% Thus, the latency can be as slow as 100\,ms, without any noticeable impact.
% As shown in Section~\ref{experimentalResults}, this is sufficient for setting up a stream and handling encryption keys whenever a message is to be transmitted.
% The stream does not need to be set up in advance.
% \end{itemize}

% To optimize the key exchange for real-time systems, this setup time needs to be as short as possible:
% \begin{equation}
% \label{equ:tAuthMin}
% \begin{split}
% 	\argmin_{\tau_{\mathrm{auth}} > 0} \tau_{\mathrm{auth}}
% \end{split}
% \end{equation}

This concludes the stream authorization and the design of the framework.
In the following section, we verify our framework by means of a formal verification tool for security protocols.

==> content/scenarios.tex <==
%!TEX root = ../lightweightAuthentication.tex
\section{Scenarios}
\label{sec:Scenarios}
\numberofpages{2-3}
Throughout its lifetime, every vehicle experiences a certain set of scenarios, which are divergent from the standard driving behavior.
To ensure full operational capabilities, these situations need to be handled in the lightweight authentication framework.
In this section, we describe these special scenarios, as well as the support by the lightweight authentication framework to handle these.
\todophilipp{change of certificates needs to be here also, in case ECU certs are not eternally valid}

\subsection{System Setup}
\label{sec:Scen_SystemSetup}
% \todophilipp{How can the system (car) be built in the factory? Secure environment?, generation of certificates on ECUs, exchange of certs, programming of gateway, ...}
The first non-standard situation in terms of authentication the vehicle experiences is the manufacturing of its components and the assembly of the same in the factory.
At some point in this process, the \glspl{ECU} and security module are bare and do not have any security certificates.
The devices are most vulnerable at this point, as no protected communication can be established.
Thus, the security of all devices in the following process is essential to guarantee the security of the following tasks.

The devices require certificates, which are generated by the respective \gls{CA} and transmitted (via a secure connection) to a programming computer.
This computer then programs the certificates into the devices.
In this setup, the programming connection between computer and device needs to be secured both digitally and physically.
This connection can be placed in the manufacturing process of the device, ideally at the first start of the device (\gls{ECU} or security module).

In addition to the device certificates, the security module also requires an \gls{ACL} containing all message streams, their sending and receiving \glspl{ECU}, as well as a list with all \glspl{ECU} built into the vehicle.
With these lists, the security module can verify if all \glspl{ECU} are correctly built into the vehicle and which \glspl{ECU} have access to which streams.
These lists can be automatically generated by the configuration management of the \gls{OEM} and need to be signed with the corresponding certificate.

\subsection{Vehicle Start}
\label{sec:Scen_VehicleStart}
When the vehicle is first started up in manufacturing, all \glspl{ECU} need to be authenticated for the first time.
This can take a significant amount of time, if all \glspl{ECU} are requesting authentication at the same time (see Section~\ref{sec:Results}).
Here, the security module can also check the existence of all expected \glspl{ECU} and ensure that no wrong \glspl{ECU} are built into the vehicle.
After all \glspl{ECU} are authenticated, all required streams can the authorized.

At subsequent starts of the vehicle, not every \gls{ECU} requires to be authenticated at the same time.
Authentication is only performed in fixed intervals, plus a random component in defined bounds.
Thus, generally only stream authorization for immediately required streams needs to be performed at subsequent vehicle starts.

\subsection{Vehicle Service}
\label{sec:Scen_VehicleService}
An additional challenge for an authentication mechanisms that relies on fixed architectures is the exchange of devices.
In the automotive context, this might happen when a damaged \gls{ECU} needs to be replaced.
The process to replace \glspl{ECU} is depicted in Fig.~\ref{fig:exchangeECUs}.
After mutual authentication (see Section~\ref{sec:Design_ECUAuthentication}) of security module and workshop (Fig.~\ref{fig:exchangeECUs} (1) \& (2)), which might include updates of the respective \glspl{CRL}, the actual process of \gls{ECU} exchange beings.
This process is initiated by the workshop requesting removal of a damaged \gls{ECU} and, after validation of the certificate, is followed by the confirmation of the security module (Fig.~\ref{fig:exchangeECUs} (3) \& (4)).
Later, the certificate of the replacement \gls{ECU} is added to the security module by a message from the workshop (Fig.~\ref{fig:exchangeECUs} (5)).
After successful verification of the workshop certificate and addition of the \gls{ECU}, a confirmation message is sent to the workshop (Fig.~\ref{fig:exchangeECUs} (6)).

It is most important that all messages in this exchange are signed to ensure that only the allowed participants can pursue these steps.
To avoid further misuse of this function, a two factor authentication, as known from banking and other systems on the internet, could be introduced between steps (3) and (4).
This could be implemented e.g. via SMS to the vehicle owner, thus informing the vehicle owner of and requesting his permission for the exchange of an \gls{ECU}.

A special case of an \gls{ECU} exchange is the exchange of the security module.
In this case, the process in Fig.~\ref{fig:exchangeECUs} needs to be repeated with every \gls{ECU}, instead of the security module.
In this context, the certificate of the security module to be removed is overwritten with the certificate of the new security module on every \gls{ECU}.

\begin{figure}
	\centering
	\includegraphics[width=\hsize]{./diagrams/exchangeOfECUs.pdf}
	\caption{High-level description of the replacement of \glspl{ECU} in workshop situations. The initial authentication (steps (1) \& (2)) can be performed like the \gls{ECU} authentication. Consecutively, \glspl{ECU} can be removed, and new \glspl{ECU} can be added to the security module. An extension with two factor authentication between steps (3) and (4) would increase security against misuse significantly.}
	\label{fig:exchangeECUs}
\end{figure}

\subsection{Firmware updates}
\label{sec:Scen_OTA}
In connected vehicles, the possibility of \acrfull{OTA} updates is becoming increasingly important.
For not-connected vehicles, firmware updates are usually performed at workshops.
By being able to update software at any point in time, the number of visits to repair shops, as well as the downtime of the vehicle are reduced significantly.
However, firmware updates, especially \gls{OTA} updates, can form a considerable insecurity, if not secured properly.
\gls{OTA} updates are available in some of the vehicles in the market today.
In these cases, signed firmware updates are used and are verified by the receiving \gls{ECU}, if possible.
If the receiving \gls{ECU} does not have the computational power to verify the certificate, an additional element, such as the cellular gateway can perform this task.
In this case, the programming of the \gls{ECU} is performed over the internal networks, based on trust.
The only security measure against illegitimate firmware updates from the \gls{CAN} bus is usually a simple password that can often be recovered from the tuner community \cite{koscher2010}.
With our proposed lightweight authentication framework, we can replace this simple password with our authentication scheme and ensure that the firmware update is authenticated all the way until the \gls{ECU}.

All firmware updates are run via the security module, which in turn verifies the identity of the sender and the validity of the firmware signature for the \gls{ECU}.
The firmware is signed with the private key of the sending instance, which is certified in the tree of trust (see Section~\ref{sec:CRL}).
After successful verification, the security module triggers the programming of the \gls{ECU}.
To ensure a maximum of security, the \gls{ECU} authentication (see Section~\ref{sec:Design_ECUAuthentication}), including the re-validation of the security module certificate, is started as soon as a reprogramming command is received and before a new firmware is accepted.
After successful authentication of both the security module and the \gls{ECU}, the update is installed on the \gls{ECU}.
